A Reexamination of the Communication Bandwidth Cost Analysis of A Parallel Recursive Algorithm for Solving Triangular Systems of Linear Equations

This paper presents a reexamination of the research paper titled "Communication-Avoiding Parallel Algorithms for \proc{TRSM}" by Wicky et al. We focus on the communication bandwidth cost analysis presented in the original work and identify potential issues that require clarification or revision. The problem at hand is the need to address inconsistencies and miscalculations found in the analysis, particularly in the categorization of costs into three scenarios based on the relationship between matrix dimensions and processor count. Our findings contribute to the ongoing discourse in the field and pave the way for further improvements in this area of research.

==> concl.tex <==
\secput{concl}{Conclusion}

In this paper, we have presented a detailed technical review of the \func{COnfLUX} algorithm and its associated analyses as reported in the work of Kwasniewski et al \cite{KwasniewskiKaBe21}. Our critique highlights several potential issues that could impact the validity of the original work's claims. We believe that our findings could contribute to a more thorough understanding of the \func{COnfLUX} algorithm and the challenges associated with developing optimized matrix factorization algorithms. We hope that our critique will stimulate further research and discussion in this area. 

\section*{Acknowledgement}

We would like to thank the authors of the original paper for their contributions to the field, and we appreciate the opportunity to discuss and critique their work. Our intention is not to diminish the value of their research, but rather to contribute to the ongoing scientific discourse and to the shared goal of improving the performance and efficiency of matrix factorization algorithms. 


==> intro.tex <==
\secput{intro}{Introduction}

Matrix factorizations play a crucial role in various scientific computations. In the realm of high-performance computing, there has been a significant interest in developing optimized algorithms for factorizations. Kwasniewski et al. \cite{KwasniewskiKaBe21} have made a notable contribution to this field with their work on the \func{COnfLUX} algorithm, a variant of the 2.5D LU factorization algorithm with tournament pivoting. Their paper presents a theoretical framework for the algorithm and includes experimental validation, as well as a derivation of a matching lower bound.

However, upon careful examination, we have identified several potential issues in their paper. This article aims to provide a comprehensive technical re-examination of the \func{COnfLUX} algorithm and its associated analyses, addressing these identified issues. Specifically, our analysis investigates the estimation of the upper bound in the \func{COnfLUX} algorithm, scrutinizes its experimental methods, and examines the corresponding lower bound.

\paragrf{Identified Issues}

Through a meticulous review of the \func{COnfLUX} algorithm and its accompanying analyses in the original paper, we have pinpointed potential issues in the following areas, listed in order of significance:

\begin{enumerate}
    \item The upper bound of the \func{COnfLUX} algorithm: We have observed a discrepancy between the authors' analyses and the actual communication bandwidth costs incurred by the algorithm. Specifically, the utilization of a 1D decomposition for certain regions (for panel factorization and \proc{TRSM}) in the algorithm may not fully harness the communication capabilities of \emph{all} processors, resulting in an underestimation of the bandwidth cost.
    \item The empirical methods: Upon examining the original code base \footnote{Snapshot taken on May 29, 2023 from \href{https://github.com/eth-cscs/conflux}{https://github.com/eth-cscs/conflux}}, we have discovered that the authors only tested certain processor grid configurations and did not evaluate the \co{} configurations stated in the paper. This discrepancy has the potential to affect the validity of the claim regarding the communication optimality of the algorithm proposed in the paper.
    \item The derivation of the lower bound: The lower bound derivation may oversimplify the matter by not considering the fact that in parallel computation, the total amount of I/O operations typically increases proportionally to the number of processors, which is often asymptotically larger than in sequential computation.
\end{enumerate}


